A Random-Player Game and Derangement Numbers

Consider the following game between a random player R and a deterministic player D. There is a pile of n elements at the beginning. The rules for playing are as follows: In each turn of R, if the pile contains exactly m elements, R removes k elements from the pile, where k is independently identically distributed from {1, . . . , m}. In each turn of D, D removes only one element. The winner is the player that, at the end of its round, has no elements remaining. R starts first to play. This short paper shows that Dn, which is defined as the probability of D winning the game (when is initialized with n elements), approaches 1/e when n increases; and more specifically, Dn = dn/n!, where dn is the n-th derangement number.

==> not_for_publication.tex <==
\section{Not for publication:}
Let denote $Z_n$ the number of steps $\mathfrak{R}$ takes in a game initialized with $n$ elements. 
Let now calculate $\mathbb{E}(Z_n)$ in a recursive way:

\begin{equation}
\begin{split}
    \mathbb{E}(Z_n) &= 1 + \frac{1}{n}\sum_{k=1}^{n-2}\mathbb{E}(Z_{n-k-1}) + \frac{1}{n} \cdot 0 + \frac{1}{n} \cdot 0 \\
    &= 1 + \frac{1}{n}\sum_{k=1}^{n-2}\mathbb{E}(Z_{k}) = 1 + \frac{1}{n}\sum_{k=1}^{n-3}\mathbb{E}(Z_{k}) + \frac{1}{n}\mathbb{E}(Z_{n-2}) \\
    &= 1 + \frac{n-1}{n}\biggl(\mathbb{E}(Z_{n-1})-1\biggl) + \frac{1}{n}\mathbb{E}(Z_{n-2}) \\
    &= \mathbb{E}(Z_{n-1}) + \frac{1}{n}\biggl(1-\mathbb{E}(Z_{n-1})+\mathbb{E}(Z_{n-2})\biggl)   
\end{split} \label{eq11} \tag{11}
\end{equation}

Now let denote $Q_n=Z_n-Z_{n-1}$. From Equation (\ref{eq11}) we get:

\begin{equation}
\begin{split}
    n\mathbb{E}(Q_n) & = 1-\mathbb{E}(Q_{n-1})\\  
\end{split} \label{eq12} \tag{12}
\end{equation}
